Efficient data augmentation for multivariate probit models with panel data: An application to general practitioner decision-making about contraceptives

This article considers the problem of estimating a multivariate probit model in a panel data setting with emphasis on sampling a high-dimensional correlation matrix and improving the overall efficiency of the data augmentation approach. We reparameterise the correlation matrix in a principled way and then carry out efficient Bayesian inference using Hamiltonian Monte Carlo. We also propose a novel antithetic variable method to generate samples from the posterior distribution of the random effects and regression coefficients, resulting in significant gains in efficiency. We apply the methodology by analysing stated preference data obtained from Australian general practitioners evaluating alternative contraceptive products. Our analysis suggests that the joint probability of discussing combinations of contraceptive products with a patient shows medical practice variation among the general practitioners, which indicates some resistance to even discuss these products, let alone recommend them.

==> estimates.tex <==
\section{Posterior means of the patient fixed effects in the Australian GP data} \label{app:estimation result patient}


\begin{table}[ht!]
\centering
\begin{tabular}{|c|rrrrrrrr|}
\hline
\multirow{2}{*}{Variable} & \multicolumn{8}{c|}{Product} \\ \cline{2-9}
 & \multicolumn{1}{c}{1}   & \multicolumn{1}{c}{2}   & \multicolumn{1}{c}{3}   & \multicolumn{1}{c}{4}   & \multicolumn{1}{c}{5}   & \multicolumn{1}{c}{6}   & \multicolumn{1}{c}{7}   & \multicolumn{1}{c|}{8}   \\ \hline
Intercept & \cellcolor{gray!25}1.4026  & \cellcolor{gray!25}-1.2448 & -0.3887 & \cellcolor{gray!25}1.1099  & \cellcolor{gray!25}-2.4041 & -0.1309 & \cellcolor{gray!25}-1.7113 & 0.6777  \\
dagegp1   & \cellcolor{gray!25}0.1974  & -0.1334 & 0.0110  & 0.0752  & \cellcolor{gray!25}-0.5025 & -0.0202 & \cellcolor{gray!25}-0.2892 & 0.0644  \\
dagegp3   & -0.1309 & 0.0614  & -0.0620 & -0.0003 & \cellcolor{gray!25}0.3161  & -0.0032 & 0.0857  & 0.0109  \\
dagegp4   & \cellcolor{gray!25}-0.3881 & \cellcolor{gray!25}0.1814  & \cellcolor{gray!25}-0.2384 & -0.1042 & \cellcolor{gray!25}0.8045  & -0.0268 & \cellcolor{gray!25}0.3775  & 0.0017  \\
drfe2     & -0.0430 & 0.0008  & -0.0372 & -0.0140 & 0.0434  & -0.0189 & -0.0471 & 0.0070  \\
drfe3     & \cellcolor{gray!25}-0.2479 & -0.0529 & 0.0285  & 0.0762  & 0.0914  & 0.1058  & -0.0275 & \cellcolor{gray!25}0.1353  \\
drfe4     & -0.0199 & 0.1012  & -0.0094 & 0.0513  & 0.0666  & 0.0723  & -0.0719 & 0.0054  \\
dbleed1   & 0.0500  & \cellcolor{gray!25}-0.1327 & 0.0604  & -0.0887 & \cellcolor{gray!25}0.3982  & -0.0249 & \cellcolor{gray!25}-0.5218 & \cellcolor{gray!25}-0.2285 \\
dbleed2   & 0.0163  & -0.0748 & 0.0217  & -0.0227 & 0.0068  & 0.0397  & -0.0821 & -0.0248 \\
dbp1      & -0.0591 & 0.0000  & -0.0303 & 0.0288  & 0.0034  & 0.0306  & -0.0235 & \cellcolor{gray!25}-0.1427 \\
dbp3      & \cellcolor{gray!25}-0.9902 & \cellcolor{gray!25}0.2436  & 0.0060  & 0.0128  & \cellcolor{gray!25}0.2350  & \cellcolor{gray!25}-0.2954 & \cellcolor{gray!25}0.2541  & 0.0355  \\
drel1     & 0.0426  & -0.0107 & -0.0933 & -0.0022 & \cellcolor{gray!25}0.1565  & 0.0293  & 0.0290  & \cellcolor{gray!25}-0.3945 \\
drel3     & -0.0144 & 0.0272  & -0.0206 & 0.0004  & -0.0261 & 0.0086  & -0.0185 & 0.0190  \\
drel4     & -0.0916 & 0.0869  & 0.0691  & -0.0006 & -0.0094 & 0.0285  & 0.0033  & \cellcolor{gray!25}-0.2036 \\
dchild1   & \cellcolor{gray!25}-1.7332 & \cellcolor{gray!25}1.3001  & -0.0078 & -0.0903 & \cellcolor{gray!25}0.9163  & \cellcolor{gray!25}-0.9867 & \cellcolor{gray!25}0.5286  & -0.0371 \\
dchild2   & -0.0462 & 0.0350  & -0.0626 & -0.0410 & \cellcolor{gray!25}0.9787  & -0.0504 & \cellcolor{gray!25}0.5930  & -0.0539 \\
dfut1     & \cellcolor{gray!25}-0.3189 & -0.0043 & \cellcolor{gray!25}0.1956  & 0.0249  & \cellcolor{gray!25}0.6284  & -0.0775 & \cellcolor{gray!25}0.2036  & -0.1144 \\
dfut2     & \cellcolor{gray!25}-0.2846 & \cellcolor{gray!25}0.1912  & \cellcolor{gray!25}-0.2151 & \cellcolor{gray!25}-0.1990 & -0.0067 & 0.0366  & -0.1458 & 0.0115  \\
dfut4     & \cellcolor{gray!25}-0.3581 & 0.0496  & 0.0475  & 0.0106  & \cellcolor{gray!25}0.2882  & 0.0059  & 0.0128  & 0.0312  \\
dpil1     & \cellcolor{gray!25}0.4713  & \cellcolor{gray!25}0.3618  & -0.0934 & \cellcolor{gray!25}-0.2596 & -0.0112 & -0.0316 & -0.0441 & -0.0278 \\
dpil3     & \cellcolor{gray!25}-0.1822 & \cellcolor{gray!25}-0.2448 & 0.0300  & 0.0612  & 0.0552  & 0.0351  & 0.0469  & 0.0816  \\
dwt1      & 0.0815  & 0.0368  & \cellcolor{gray!25}-0.2582 & -0.0616 & 0.0318  & 0.0640  & -0.0127 & 0.0833  \\
dcomp2    & \cellcolor{gray!25}-0.3389 & \cellcolor{gray!25}-0.1969 & \cellcolor{gray!25}0.2133  & 0.0628  & \cellcolor{gray!25}0.2300  & -0.0034 & \cellcolor{gray!25}0.3100  & -0.0164 \\
dpay2     & -0.0245 & -0.0540 & -0.0202 & -0.0029 & 0.0080  & 0.0603  & 0.0072  & 0.0075  \\
dpay3     & 0.0321  & -0.0631 & -0.0683 & -0.0167 & -0.0365 & \cellcolor{gray!25}0.2909  & -0.0173 & -0.0046 \\
dsmk2     & \cellcolor{gray!25}-0.2666 & -0.0118 & -0.0266 & -0.0129 & -0.0038 & 0.0422  & 0.0867  & 0.0308  \\
dsmk3     & \cellcolor{gray!25}-0.5183 & -0.0143 & 0.0125  & 0.0248  & 0.0144  & -0.0531 & 0.0461  & 0.0332  \\ \hline
\end{tabular}
\caption{Regression coefficient posterior mean estimates for the attributes of a female patient for various products in the contraceptive discussion data.  Parameters whose 90\% credible interval does not include 0 are shown in grey.}
\label{table:estimation result for women attributes}
\end{table}


\section{Posterior means of the GP fixed effects in the Australian GP data} \label{app:estimation result GP}


\begin{table}[ht!]
\centering
\begin{tabular}{|c|rrrrrrrr|}
\hline
\multirow{2}{*}{Variable} & \multicolumn{8}{c|}{Product} \\ \cline{2-9}
                                                                      & \multicolumn{1}{c}{1}   & \multicolumn{1}{c}{2}   & \multicolumn{1}{c}{3}   & \multicolumn{1}{c}{4}   & \multicolumn{1}{c}{5}   & \multicolumn{1}{c}{6}   & \multicolumn{1}{c}{7}   & \multicolumn{1}{c|}{8}   \\ \hline
Female                                                                         & -0.0643                  & 0.0254                   & \cellcolor{gray!25}-0.4392                  & 0.0716                   & 0.0375                   & \cellcolor{gray!25}0.6089                   & \cellcolor{gray!25}-0.4569                  & -0.0248                  \\ \hline
Fellow                                                                         & -0.0182                  & -0.0990                  & 0.0682                   & 0.0375                   & 0.2107                   & 0.1086                   & -0.1452                  &  -0.0091                  \\  \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Family\\ planning\end{tabular}}     & \multirow{2}{*}{-0.0004} & \multirow{2}{*}{-0.0160} & \multirow{2}{*}{-0.1220} & \multirow{2}{*}{0.2292}  & \multirow{2}{*}{0.0446}  & \multirow{2}{*}{0.0360}  & \multirow{2}{*}{-0.0321} & \multirow{2}{*}{-0.0133} \\
                                                                               &                          &                          &                          &                          &                          &                          &                          &                          \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Bulk-\\ bill\end{tabular}}          & \multirow{2}{*}{-0.0199} & \multirow{2}{*}{-0.0372} & \multirow{2}{*}{0.0425}  & \multirow{2}{*}{-0.0389} & \multirow{2}{*}{-0.0594} & \multirow{2}{*}{ 0.0035} & \multirow{2}{*}{0.0503}  & \multirow{2}{*}{0.0060}  \\
                                                                               &                          &                          &                          &                          &                          &                          &                          &                          \\ \hline
Age                                                                            & 0.0087                   & 0.0079                   & \cellcolor{gray!25}0.0205                   & -0.0064                  & \cellcolor{gray!25}0.0176                   & -0.0043                  & 0.0090                  & -0.0101                  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Australian\\ graduate\end{tabular}} & \multirow{2}{*}{0.0835}  & \multirow{2}{*}{0.0569}  & \multirow{2}{*}{-0.0080}  & \multirow{2}{*}{0.3457}  & \multirow{2}{*}{0.0989}  & \multirow{2}{*}{-0.2348} & \multirow{2}{*}{-0.0933} &  \cellcolor{gray!25} \\
                                                                               &                          &                          &                          &                          &                          &                          &                          &  \multirow{-2}{*}{\cellcolor{gray!25}0.5586}                        \\ \hline
Urban                                                                          & -0.0947                  & 0.0072                   & 0.0693                   & -0.0073                  & 0.0112                  & 0.0040                   & -0.0285                   & 0.1814                   \\ \hline
\end{tabular}
\caption{Regression coefficient posterior mean estimates for the GP fixed effects for various products in the contraceptive discussion data.  Parameters whose 90\% credible interval does not include 0 are shown in grey.}
\label{table:estimation result for doctors fixed effects}
\end{table}


\newpage
\section{Posterior means of the parameters in \texorpdfstring{$\bR$}{bReps}} \label{app:correlation}


\begin{table}[ht!]
\centering
\begin{tabular}{|c|c|c|}
\hline
Parameter & Posterior Mean & 95\% Credible Interval \\
\hline
$r_{21}$ & -0.1157   & (-0.2058, -0.0251)     \\
$r_{31}$ & -0.0502   & (-0.1446, { }0.0451)   \\
$r_{32}$ & { }0.1617 & ({ }0.0707, { }0.2506) \\
$r_{41}$ & -0.0481   & (-0.1512, { }0.0532)   \\
$r_{42}$ & { }0.0454 & (-0.0578, { }0.1512)   \\
$r_{43}$ & { }0.5891 & ({ }0.5151, { }0.6577) \\
$r_{51}$ & -0.2354   & (-0.3223, -0.1467)     \\
$r_{52}$ & -0.0255   & (-0.1203, { }0.0695)   \\
$r_{53}$ & { }0.1759 & ({ }0.0822, { }0.2657) \\
$r_{54}$ & { }0.2424 & ({ }0.1431, { }0.3398) \\
$r_{61}$ & { }0.4721 & ({ }0.3930, { }0.5472) \\
$r_{62}$ & -0.2702   & (-0.3572, -0.1810)     \\
$r_{63}$ & { }0.0144 & (-0.0753, { }0.1038)   \\
$r_{64}$ & { }0.0358 & (-0.0646, { }0.1367)   \\
$r_{65}$ & -0.0695   & (-0.1629, { }0.0266)   \\
$r_{71}$ & -0.2054   & (-0.3068, -0.1028)     \\
$r_{72}$ & -0.0540   & (-0.1559, { }0.0499)   \\
$r_{73}$ & { }0.1849 & ({ }0.0810, { }0.2877) \\
$r_{74}$ & { }0.1877 & ({ }0.0747, { }0.2973) \\
$r_{75}$ & { }0.5185 & ({ }0.4288, { }0.6016) \\
$r_{76}$ & -0.0051   & (-0.1138, { }0.1014)   \\
$r_{81}$ & -0.0196   & (-0.1147, { }0.0749)   \\
$r_{82}$ & -0.0491   & (-0.1412, { }0.0440)   \\
$r_{83}$ & { }0.0205 & (-0.0704, { }0.1091)   \\
$r_{84}$ & { }0.1044 & ({ }0.0059, { }0.2009) \\
$r_{85}$ & -0.0788   & (-0.1701, { }0.0131)   \\
$r_{86}$ & { }0.1841 & ({ }0.0930, { }0.2753) \\
$r_{87}$ & { }0.2046 & ({ }0.1036, { }0.3040) \\ \hline
\end{tabular}
\caption{Posterior mean estimates of the elements in the correlation matrix $\bR$ of the errors terms with their 95\% credible intervals.}
\label{table:correlation}
\end{table}


\newpage
\section{Posterior means of the parameters in \texorpdfstring{$\Sig_{\ba}$}{Sigba}} \label{app:covariance}


\begin{table}[ht!]
\centering
\begin{tabular}{|c|c|c|}
\hline
Parameter & Posterior Mean & 95\% Credible Interval \\
\hline
$\s^2_{\a_1}$ & { }0.5147  & ({ }0.3630, 0.7095) \\
$\s^2_{\a_2}$ & { }0.6492  & ({ }0.4745, 0.8690) \\
$\s^2_{\a_3}$ & { }1.3021  & ({ }0.9554, 1.7634) \\
$\s^2_{\a_4}$ & { }1.5329  & ({ }1.0905, 2.1402) \\
$\s^2_{\a_5}$ & { }1.0586  & ({ }0.7785, 1.4112) \\
$\s^2_{\a_6}$ & { }1.4533  & ({ }1.0695, 1.9627) \\
$\s^2_{\a_7}$ & { }1.9449  & ({ }1.3741, 2.7053) \\
$\s^2_{\a_8}$ & { }1.2432  & ({ }0.8962, 1.6945) \\
$\s_{(\a_2, \a_1)}$ & { }0.3009  & ({ }0.1813, 0.4417) \\
$\s_{(\a_3, \a_1)}$ & { }0.2733  & ({ }0.1148, 0.4542) \\
$\s_{(\a_3, \a_2)}$ & { }0.3026  & ({ }0.1314, 0.5004) \\
$\s_{(\a_4, \a_1)}$ & { }0.2481  & ({ }0.0731, 0.4489) \\
$\s_{(\a_4, \a_2)}$ & { }0.2659  & ({ }0.0681, 0.4870) \\
$\s_{(\a_4, \a_3)}$ & { }0.2525  & (-0.0200, 0.5434)   \\
$\s_{(\a_5, \a_1)}$ & { }0.0764  & (-0.0677, 0.2272)   \\
$\s_{(\a_5, \a_2)}$ & { }0.1866  & ({ }0.0322, 0.3566) \\
$\s_{(\a_5, \a_3)}$ & -0.0177    & (-0.2376, 0.2022)   \\
$\s_{(\a_5, \a_4)}$ & { }0.5141  & ({ }0.2705, 0.8058) \\
$\s_{(\a_6, \a_1)}$ & { }0.2012  & ({ }0.0305, 0.3969) \\
$\s_{(\a_6, \a_2)}$ & { }0.2195  & ({ }0.0360, 0.4232) \\
$\s_{(\a_6, \a_3)}$ & { }0.1101  & (-0.1427, 0.3672)   \\
$\s_{(\a_6, \a_4)}$ & { }0.2469  & (-0.0342, 0.5528)   \\
$\s_{(\a_6, \a_5)}$ & { }0.2856  & ({ }0.0539, 0.5430) \\
$\s_{(\a_7, \a_1)}$ & { }0.0611  & (-0.1420, 0.2722)   \\
$\s_{(\a_7, \a_2)}$ & { }0.2400  & ({ }0.0277, 0.4768) \\
$\s_{(\a_7, \a_3)}$ & { }0.2573  & (-0.0378, 0.5871)   \\
$\s_{(\a_7, \a_4)}$ & -0.2164    & (-0.5979, 0.1113)   \\
$\s_{(\a_7, \a_5)}$ & { }0.0148  & (-0.2596, 0.2956)   \\
$\s_{(\a_7, \a_6)}$ & { }0.2915  & (-0.0194, 0.6297)   \\
$\s_{(\a_8, \a_1)}$ & { }0.2570  & ({ }0.0982, 0.4404) \\
$\s_{(\a_8, \a_2)}$ & { }0.3344  & ({ }0.1562, 0.5423) \\
$\s_{(\a_8, \a_3)}$ & { }0.0750  & (-0.1594, 0.3157)   \\
$\s_{(\a_8, \a_4)}$ & { }0.2315  & (-0.0290, 0.5223)   \\
$\s_{(\a_8, \a_5)}$ & { }0.2537  & ({ }0.0449, 0.4889) \\
$\s_{(\a_8, \a_6)}$ & { }0.4904  & ({ }0.2432, 0.7802) \\
$\s_{(\a_8, \a_7)}$ & { }0.4139  & ({ }0.1235, 0.7563) \\ \hline
\end{tabular}
\caption{Posterior mean estimates of the elements in the covariance matrix $\Sig_{\ba}$ of the random effects with their 95\% credible intervals.  The variance parameter in $\Sig_{\ba}$ is denoted by $\s^2_{\a_i}$ while the $(i,j)$-th covariance parameter is given by $\s_{(\a_i, \a_j)}$.}
\label{table:covariance}
\end{table}

==> px.tex <==
\section{Parameter expansion for the MVP model} \label{app:parameter} % 588


We first describe the parameter expansion (PX) strategy in \cite{talhouk2012efficient} for the MVP % 589
model based on the marginally uniform prior on $\bR$ of \cite{barnard2000modeling}.  We then illustrate % 590
the extension of this method to the panel data setting where the resulting sampler fails to % 591
converge to the correct posterior distribution. % 592

Consider the MVP model as in Section~\ref{sec:multivariate}, but without the random effects, % 593
\begin{gather}
\by^*_{i} = \bB \bx_{i} + \beps_{i}, \\
\beps_{i} = (\eps_{1,i}, \dotsc, \eps_{D,i})^\top \stackrel{iid}{\sim} \N({\bf 0}, \bR),
\end{gather}
for $i=1,\dotsc,n$.  The posterior density of interest given the set of observed discrete outcomes % 594
$\by=(\by_1,\dotsc,\by_n)$ and prior distribution $p(\bB, \bR)$ is % 595
\begin{equation}
\pi(\by^*, \bB, \bR|\by) \propto p(\by|\by^*, \bB, \bR)p(\by^*|\bB, \bR)p(\bB, \bR).
\label{eqn:MVP posterior}
\end{equation}
By taking advantage of the non-identifiability of the regression parameter $\bB$ when $\bR$ is % 596
not set to be a correlation matrix, \cite{talhouk2012efficient} introduce an expansion parameter % 597
$\bD=\diag(\d_1, \dotsc, \d_D)$ and define a new set of latent variables $\bz^*_i=\bD\by^*_i, i=1, \dotsc, n$ such that % 598
the posterior density under this transformation is % 599
\begin{equation}
\pi(\bz^*, \bB, \bR, \bD|\by) \propto p(\by|\bz^*, \bB, \bR, \bD)p(\bz^*|\bB, \bR, \bD)p(\bB, \bR,\bD),
\label{eqn:MVP PX posterior}
\end{equation}
where $\bz^*=(\bz^*_1, \dotsc, \bz^*_n)$.  The marginal posterior distribution of $(\bB, \bR)$ in (\ref{eqn:MVP PX posterior}) is the same as % 600
(\ref{eqn:MVP posterior}) provided that the marginal prior of $p(\bB, \bR,\bD)$ is $p(\bB, \bR)$.  Using the prior distribution % 601
on $\bR$ in (\ref{eqn:marginally uniform prior}) with $\nu=D+1$ and choosing % 602
\begin{equation}
\d_i^2 \stackrel{iid}{\sim} \mathcal{IG}((D+1)/2, \bR^{-1}(i,i)/2),
\label{eqn:inverse gamma}
\end{equation}
where $\bR^{-1}(i,i)$ is the $i$-th diagonal entry of $\bR$, the covariance matrix $\Sig_{\beps}=\bD \bR \bD$ is shown % 603
to have an $\mathcal{IW}(D+1, \bm{I})$ distribution.  With this reparameterisation of the constrained $\bR$ % 604
into an unconstrained $\Sig_{\beps}$, posterior sampling from the conditional posterior distribution % 605
$\pi(\bB, \bR, \bD|\bz^*, \by)$ can be circumvented by a change of variables technique.  That is, by letting % 606
$\Sig_{\beps}=\bD \bR \bD$ and $\bm{\g}=\bD \bB$, iterates from the posterior distribution in (\ref{eqn:MVP posterior}) can be obtained % 607
by the following steps: % 608
\begin{enumerate}
\item Sample $\by^*$ from a truncated multivariate normal distribution (Step 1 in Appendix~\ref{app:sampling scheme}). % 609
\item Sample $\bD$ following (\ref{eqn:inverse gamma}) and set $\bz_i^* = \bD \by_i^*, i=1,\dotsc,n$. % 610
\item Sample $(\bm{\g}, \Sig_{\beps}) \sim \pi(\bm{\g}, \Sig_{\beps}|\bz^*, \by)$. % 611
\item Set $\bB=\bD^* \bm{\g}, \bR=\bD^* \Sig_{\beps} \bD^*$ and $\by_i^*=\bD^* \bz_i^*, i=1, \dotsc, n$ where $\bD^* = \diag(\Sig_{\beps})^{-1/2}$. % 612
\end{enumerate}

The posterior density of the MVP model with random effects in (\ref{eqn:MVP})--(\ref{eqn:latent}), on the other % 613
hand, is % 614
\begin{equation}
\begin{aligned}
\pi(\by^*, \bB, \bR, \ba_{1:P}, \Sig_{\ba}|\by) \propto & p(\by|\by^*, \bB, \bR, \ba_{1:P}, \Sig_{\ba}) \times \\
& p(\by^*|\bB, \bR, \ba_{1:P}, \Sig_{\ba})p(\ba_{1:P}|\Sig_{\ba})p(\bB, \bR, \Sig_{\ba}).
\end{aligned}
\label{eqn:MVP with RE posterior}
\end{equation}
Following \cite{talhouk2012efficient}, we define new sets of latents variables $\bz^*_{it} = \bD \by^*_{it}$ and % 615
$\bm{w}_i = \bD \ba_i$ for $i=1,\dotsc,P$ and $t=1,\dotsc,T$, which gives the new posterior density as % 616
\begin{equation}
\begin{aligned}
\pi(\bz^*, \bB, \bR, \bm{w}_{1:P}, \Sig_{\ba}, \bD|\by) \propto & p(\by|\bz^*, \bB, \bR, \bm{w}_{1:P}, \Sig_{\ba}, \bD) p(\bz^*|\bB, \bR, \bm{w}_{1:P}, \Sig_{\ba}, \bD) \times \\ &p(\bm{w}_{1:P}|\Sig_{\ba}, \bD)p(\bB, \bR, \Sig_{\ba}, \bD),
\end{aligned}
\label{eqn:MVP with RE PX posterior}
\end{equation}
where $\bz^*=(\bz_{it};i=1, \dotsc,P, t=1, \dotsc, T)$ and $\bm{w}_{1:P}=(\bm{w}_1, \dotsc, \bm{w}_P)$.  Assuming a conjugate % 617
prior on $\Sig_{\ba}$, we then generate the samples from the posterior distribution in (\ref{eqn:MVP with RE PX posterior}) by a change % 618
of variables ($\Sig_{\beps}=\bD \bR \bD$ and $\bm{\g}=\bD \bB$) according to % 619
\begin{enumerate}
\item Sample $\by^*$ from a truncated multivariate normal distribution (Step 1 in Appendix~\ref{app:sampling scheme}). % 620
\item Sample $\ba_{1:P}$ from a multivariate normal distribution (Step 4 in Appendix~\ref{app:sampling scheme}). % 621
\item Sample $\Sig_{\ba}$ from an inverse-Wishart distribution (Step 6 in Appendix~\ref{app:sampling scheme}). % 622
\item Sample $\bD$ following (\ref{eqn:inverse gamma}) and set $\bz_{it}^* = \bD \by_{it}^*$ and $\bm{w}_i = \bD \ba_i$ for $i=1,\dotsc,P$ and % 623
$t=1,\dotsc,T$. % 624
\item Sample $(\bm{\g}, \Sig_{\beps}) \sim \pi(\bm{\g}, \Sig_{\beps}|\bz^*, \by)$. % 625
\item Set $\bB=\bD^* \bm{\g}, \bR=\bD^* \Sig_{\beps} \bD^*$ and $\by_{it}^*=\bD^* \bz_{it}^*, i=1, \dotsc, P, t=1,\dotsc,T$ where $\bD^* = \diag(\Sig_{\beps})^{-1/2}$. % 626, 627
\end{enumerate}
We choose the conjugate matrix normal prior on $\bB$, the marginally uniform prior in (\ref{eqn:marginally uniform prior}) on % 628
$\bR$ and the hierarchical inverse-Wishart prior on $\Sig_{\ba}$.  Kernel density plots comparing the % 629
posterior distribution of the variance parameter in $\Sig_{\ba}$ between the HMC algorithm and the % 630
parameter expansion technique are given in Figure~\ref{fig:hmc vs px}.  Using the posterior distribution from % 631
the HMC algorithm as a benchmark, we notice that the parameter expansion method tends to % 632
overestimate the variance of the random effects and the posterior densities are flatter.  The % 633
observed differences are due to the PX technique, not the choice of kernel density bandwidth. % 634
\begin{figure}[h!]
\onehalfspacing
\centering
\includegraphics[trim= 0.5cm 1cm 1.5cm 1.75cm,clip,width=0.75\textwidth]{hmc_vs_px_hiw}
\caption{Kernel density plots comparing the posterior density of the variance parameter $\s^2_{\a_i}$ in $\Sig_{\ba}$ between the HMC algorithm (blue solid) and the parameter expansion technique (red dashed).}
\label{fig:hmc vs px}
\end{figure}
